An alternating peak-optimization method for optimal trajectory generation of quadrotor drones

In this paper, we propose an alternating optimization method to address a time-optimal trajectory generation problem. Different from the existing solutions, our approach introduces a new formulation that minimizes the overall trajectory running time while maintaining the polynomial smoothness constraints and incorporating hard limits on motion derivatives to ensure feasibility. To address this problem, an alternating peak-optimization method is developed, which splits the optimization process into two sub-optimizations: the first sub-optimization optimizes polynomial coefficients for smoothness, and the second sub-optimization adjusts the time allocated to each trajectory segment. These are alternated until a feasible minimum-time solution is found. We offer a comprehensive set of simulations and experiments to showcase the superior performance of our approach in comparison to existing methods. A collection of demonstration videos with real drone flying experiments can be accessed at https://www.youtube.com/playlist?list=PLQGtPFK17zUYkwFT-fr0a8E49R8Uq712l .

==> Chapters/Review_of_other_methods.tex <==

Differential flatness allows the 4 dimensional trajectory to be split into four independent one-dimensional trajectories. The input for the trajectory generation will be a set of $K$ waypoints and each waypoint is defined by a position vector in three dimensional space, a yaw angle and an arrival time. 

%Using polynomials has three useful properties. Firstly, using a polynomial guarantees a smooth trajectory that the quadrotor system will be able to follow. Secondly, the trajectory can be optimised using the coefficients as decision variables in an optimization function. Thirdly, the derivatives, and thus the speeds, accelerations etc, can easily be calculated for a polynomial function of time.

% A polynomial $P$ of degree $N$ as a function of time $t$ takes the form of
% \begin{equation}
%     P(t) = p_n t^N + p_{n-1} t^{n-1} ... + p_0 = \sum_{n=0}^N p_n t^n,
% \end{equation}
% where $p_n$ are the coefficients of the polynomial.
The trajectory will be defined for each flat output and segment using a polynomial $P(t)$ of the $s$th order. The coefficients of this polynomial can then be optimised using a cost function $J$ in the form of 
\begin{equation}
    J = \int_{t=0}^{t=\tau} c_\mathrm{0} P(t)^2 + c_\mathrm{1} P^\prime(t)^2 + c_\mathrm{2} P^{\prime\prime}(t)^2 + ... + c_\mathrm{N} P^{(N)} (t)^2 dt,  
    \label{eq:minfuncP}
\end{equation}
where $c_\mathrm{N}$ are the weights of each derivative. This allows for the minimisation of the total speed, acceleration, jerk or snap present during the trajectory. Jerk and Snap are the derivatives that are most commonly optimised for. 
%The weight $c_3$ is set to one and the others are set to zero to optimise for minimum jerk trajectory and the weight $c_4$ is set to one and the others set to zero to optimise for minimum snap trajectory. 
This cost function can be rewritten into a quadratic form as 
\begin{equation}
    J_\mathrm{k} = \textbf{p}_\mathrm{\textbf{k}}^\top \textbf{Q}_\mathrm{\textbf{k}} \textbf{p}_\mathrm{\textbf{k}},
\end{equation}
where $\textbf{p}_\textbf{k}$ is a vector which contains the coefficients of the polynomial and $\textbf{Q}_\textbf{k}$ is the cost matrix. The computation of the cost matrix in the quadratic form was explained in \cite{Bry2015}. Trajectories are often constructed out of multiple segments, which requires an expanded cost function to include all the coefficients and cost matrices. The expanded cost function can be written in the compact form
\begin{equation}
    J = 
    \begin{bmatrix}
    \textbf{p}_\mathrm{0} \\
    \vdots \\
    \textbf{p}_\mathrm{K}
    \end{bmatrix}^\top
    \begin{bmatrix}
    \textbf{Q}_\mathrm{0}(\tau_\mathrm{0}) & & \\
    & \ddots & \\
    & & \textbf{Q}_\mathrm{K}(\tau_\mathrm{K}) \\
    \end{bmatrix}
        \begin{bmatrix}
    \textbf{p}_\mathrm{0} \\
    \vdots \\
   \textbf{p}_\mathrm{K}
    \end{bmatrix},
    \label{eq:minfunc}
\end{equation}
where $\tau$ is the segment time. 
Then the function can be solved as a regular quadratic programming problem of the form
% \begin{equation} \label{eq:mellinger_poly}
% \begin{aligned}
%     &min \hspace{5pt} J \\
%     &s.t.\textbf{A}\textbf{p}-\textbf{b} = 0,\\
% \end{aligned}
% \end{equation}

\begin{mini!}
{\textbf{p}_\mathrm{i}}
{J} {\label{eq:mellinger_poly}}{}
\addConstraint{\textbf{A}\textbf{p}-\textbf{b}}{ = 0}
\end{mini!}


where $\textbf{A}$ and $\textbf{b}$ are used to constrain the start, end or any intermediate positions, velocities or other derivatives and is also used to ensure continuity of any derivative. 

However, this method does not guarantee the minimum cost possible for the given problem, as the time segments were fixed beforehand to be able to construct the cost function. It is likely that a solution exists with lower costs for a different a different distribution of the time over the segments. It is therefore necessary to optimise the time distribution as well as the polynomial coefficients to obtain the solution with the lowest cost. 

Mellinger and Kumar \cite{Mellinger2011}(from hereon referred to as "Mellinger method") proposed an alternating optimization approach to solve it using a gradient descent method, which makes an initial guess for the segment times and optimise the polynomial coefficients. The following optimization function was formulated in \cite{Mellinger2011}.


\begin{mini!}
{t_\mathrm{i}}
{f(\textbf{t})} {\label{eq:timecost}}{}
\addConstraint{\sum t_\mathrm{i}}{ = t_\mathrm{m}}
\addConstraint{t_{\mathrm{i}}}{\geq 0}
\end{mini!}




% \begin{equation} \label{eq:timecost}
% \begin{aligned}
%     &min \hspace{5pt} f(\textbf{T}) \\
%     &s.t.\sum T_\mathrm{i} = t_\mathrm{m} \\
%     &T_i \geq 0,
% \end{aligned}
% \end{equation}
where $f()$ is the cost function with the optimised coefficients, $\textbf{t}$ is the vector containing all the segment times and $t_m$ is the total time. The generated optimal segment times were used to recompute the optimal coefficients. This was iterated several times until the cost function converges to a final value. 
When the final trajectory and time distribution is found, the total time can be decreased to obtain more aggressive motion, or it can be increased to make for safer motion. The changing of the total time while maintaining the same time distribution is called temporal scaling.

An improved method to obtain aggressive motion was proposed by Bry et al. \cite{Bry2015} (hereon referred to as "Bry method"). It eliminates the total time constrained in Eq.~(\ref{eq:timecost}) so that the total time would decrease. Then the optimization function was reformulated so that both the polynomial coefficients and the segment times are optimization variables. The cost function was expanded and a cost was placed upon the total time, which was described by
\begin{equation}
    J = 
    \begin{bmatrix}
    \textbf{p}_\mathrm{0} \\
    \vdots \\
    \textbf{p}_\mathrm{K}
    \end{bmatrix}^\top
    \begin{bmatrix}
    \textbf{Q}_\mathrm{0}(\tau_\mathrm{0}) & & \\
    & \ddots & \\
    & & \textbf{Q}_\mathrm{K}(\tau_\mathrm{K}) \\
    \end{bmatrix}
        \begin{bmatrix}
    \textbf{p}_\mathrm{0} \\
    \vdots \\
   \textbf{p}_\mathrm{K}
    \end{bmatrix}
    + c_\mathrm{t} \sum_{i=0}^K \tau_\mathrm{i},
    \label{eq:BryOpt}
\end{equation}
where $c_\mathrm{t}$ is a weighting coefficient on the total time. This would lead to an increase in total jerk or snap, but a lower total time, that results in more aggressive and faster trajectories. The weighting coefficient could be increased if a more aggressive trajectory was desired and lowered if a trajectory with less total snap was desired. 

It should be noted that the most aggressive and feasible trajectory is inherently non-smooth and would therefore not be achievable using polynomial trajectories. Some other form of optimization such as time-optimal planning is required to achieve the most aggressive trajectory possible as was demonstrated by Foehn, Romero and Scaramuzza in \cite{Foehn2021}. This approach does however require a very complex and accurate model of the drone, while the polynomial trajectories require far less information and are therefore easier to implement.

 

==> Chapters/X_Conclusion.tex <==
A new segment times optimisation method for aggressive trajectory planning was proposed. The relevant drone dynamics and the principle of differential flatness were discussed. Then the currently available methods as proposed by Mellinger and Bry were discussed. A new method to optimise the segment times allocation was proposed that focused on being consistently close to the limitation of the current system. The new and existing methods were implemented in simulation and tested on the Crazyflie platform. The combination of optimising for minimum jerk and the newly proposed peak optimisation yielded the most aggressive motion for minimal-snap or minimal-jerk trajectories. 

==> Chapters/X_Dynamics.tex <==
The drone that will be used during this project will be the Crazyflie 2.1, which consists out of a rigid frame with motors attached in a `X' pattern as can be seen in Figure \ref{fig:config}. The state of the system can be controlled by applying differential thrust across the motors. The basic dynamics were covered in \cite{Mahony2012}. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.28\textwidth]{Figures/Methods/coordinate_system.jpg}
    \caption{Coordinate frames and states of quadrotor drones \cite{coord}}
    \label{fig:config}
\end{figure}

The coordinate system includes the world frame, $W$ and the body frame $B$. The position vector that points from the world frame to the body frame is denoted by $\textbf{r}$ and the rotation matrix is denoted by $R_{WB}$. The forces and moments acting upon the drone are denoted by $\textbf{u}$ and are constructed as 
\begin{small}
\begin{equation}
\label{eq:u}
 u =     
\begin{bmatrix}
F \\
\tau_x \\ 
\tau_y \\
\tau_z 
\end{bmatrix}
= 
\begin{bmatrix}
k_F & k_F & k_F & k_F \\ 
- \frac{\sqrt{2}}{2}d k_F & - \frac{\sqrt{2}}{2}d k_F &  \frac{\sqrt{2} }{2}d k_F & \frac{\sqrt{2}}{2}d k_F \\
- \frac{\sqrt{2}}{2}d k_F &  \frac{\sqrt{2}}{2}d k_F &  \frac{\sqrt{2} }{2}d k_F & - \frac{\sqrt{2}}{2}d k_F \\
-k_M & k_M & -k_M & k_M \\ 
\end{bmatrix}
\begin{bmatrix}
\omega_1^2 \\
\omega_2^2 \\
\omega_3^2 \\
\omega_4^2 \\
\end{bmatrix}
,
\end{equation}
\end{small}
where $F$ is the combined thrust of the motors and $\tau_x$, $\tau_y$, $\tau_z$ are the generated moments about each axis, $d$ is the distance between the motor and the center of mass, $k_F$ is the force constant, $k_M$ is the torque constant and $\omega_i$ is the rotational speed of the $i_{th}$ motor. Using Newton's equation of motion results in the position motion equation

\begin{equation}
    m \Ddot{\textbf{r}} = - m g z_W + u_1 z_B,
\end{equation}
where $m$ is the mass of the drone, $g$ is the gravitational constant, $z_W$ is the z component of the world frame, $u_1$ is the combined thrust $F$ of the motors from (\ref{eq:u}) and $z_B$ is the z component of the body frame. 
The angular acceleration $\Dot{\omega}_{BW}$ can be described using the Euler equations 

\begin{equation}
    \Dot{\omega}_{BW} = I^{-1} 
    \begin{bmatrix}
    -\omega_{BW} \times I \omega_{BW} + 
    \begin{bmatrix}
    u_2 \\
    u_3 \\
    u_4 \\
    \end{bmatrix}
    \end{bmatrix},
\end{equation}
where $I$ is the moment of inertia matrix and $u_1$, $u_2$ and $u_3$ are the moments about x-axis $\tau_x$, y-axis $\tau_y$ and z-axis $\tau_z$ as described in (\ref{eq:u}) respectively. The properties of the Crazyflie 2.1 that will be used for the experiments can be found in Appendix \ref{Chapters:properties}. The mass and inertia parameters were found by Zuo in \cite{Zuo2022} and the motor constants were found by Landry in \cite{Landry2015}.


